Lifestate: Event-Driven Protocols and Callback Control Flow (Extended Version)

Developing interactive applications (apps) against event-driven software frameworks such as Android is notoriously difficult. To create apps that behave as expected, developers must follow complex and often implicit asynchronous programming protocols. Such protocols intertwine the proper registering of callbacks to receive control from the framework with appropriate application-programming interface (API) calls that in turn affect the set of possible future callbacks. An app violates the protocol when, for example, it calls a particular API method in a state of the framework where such a call is invalid. What makes automated reasoning hard in this domain is largely what makes programming apps against such frameworks hard: the specification of the protocol is unclear, and the control flow is complex, asynchronous, and higher-order. In this paper, we tackle the problem of specifying and modeling event-driven application-programming protocols. In particular, we formalize a core meta-model that captures the dialogue between event-driven frameworks and application callbacks. Based on this meta-model, we define a language called lifestate that permits precise and formal descriptions of application-programming protocols and the callback control flow imposed by the event-driven framework. Lifestate unifies modeling what app callbacks can expect of the framework with specifying rules the app must respect when calling into the framework. In this way, we effectively combine lifecycle constraints and typestate rules. To evaluate the effectiveness of lifestate modeling, we provide a dynamic verification algorithm that takes as input a trace of execution of an app and a lifestate protocol specification to either produce a trace witnessing a protocol violation or a proof that no such trace is realizable.

==> Makefile <==
######################################################################
# Makefile
#
# Makefile for LaTeX projects
######################################################################

BASE = main
PAPERS = $(BASE) $(BASE:%=%.tr)

$(PAPERS:%=%.pdf): main.short.bib bec.short.bib conference.short.bib

            #-e 's/^[ 	]*[Pp]ublisher/OPTpublisher/' \
# Generate short bib
%.short.bib: %.orig.bib
	sed -e 's/@string{SHORT/@string{/' \
            -e 's/^[ 	]*[Ee]ditor/OPTeditor/' \
            -e 's/^[ 	]*[Mm]onth/OPTmonth/' \
            -e 's/^[ 	]*[Aa]ddress/OPTaddress/' \
            -e 's/^[ 	]*[Ii]sbn/OPTisbn/' \
            -e 's/^[ 	]*[Ii]ssn/OPTissn/' \
            -e 's/^[ 	]*[Uu]rl/OPTurl/' \
            -e 's/^[ 	]*[Dd]oi/OPTdoi/' \
            -e 's/^[ 	]*[Pp]ages/OPTpages/' \
            -e 's/^[ 	]*[Cc]rossref/OPTcrossref/' \
            -e 's/^[ 	]*[Ss]eries/OPTseries/' \
            $< > $@
						
include bectex.mk


==> bectex/Makefile <==
######################################################################
# Makefile
#
# Makefile for LaTeX projects
######################################################################

BASE = main
PAPERS = $(BASE)

# Generate short bib
%.short.bib: %.orig.bib
	sed -e 's/@string{SHORT/@string{/' \
            -e 's/^[ 	]*[Ee]ditor/OPTeditor/' \
            -e 's/^[ 	]*[Mm]onth/OPTmonth/' \
            -e 's/^[ 	]*[Pp]ublisher/OPTpublisher/' \
            -e 's/^[ 	]*[Aa]ddress/OPTaddress/' \
            -e 's/^[ 	]*[Ii]sbn/OPTisbn/' \
            -e 's/^[ 	]*[Ii]ssn/OPTissn/' \
            -e 's/^[ 	]*[Uu]rl/OPTurl/' \
            -e 's/^[ 	]*[Dd]oi/OPTdoi/' \
            -e 's/^[ 	]*[Pp]ages/OPTpages/' \
            -e 's/^[ 	]*[Cc]rossref/OPTcrossref/' \
            -e 's/^[ 	]*[Ss]eries/OPTseries/' \
            $< > $@
						
include bectex.mk


==> macros.tex <==
% -*-latex-*-
\makeatletter

\newcommand{\semname}{\ensuremath{\lambda_{\text{life}}}\xspace}
\newcommand{\toolname}{Verivita\xspace}
\newcommand{\lifecyclepp}{\ensuremath{\text{lifecycle\raisebox{0.25ex}{\relsize{-1}+\!+}}}\xspace}
\newcommand{\Lifecyclepp}{\ensuremath{\text{Lifecycle\raisebox{0.25ex}{\relsize{-1}+\!+}}}\xspace}
\newcommand{\verificationtool}{Callback Verification}

\newcommand{\todoSM}[1]{\todo[inline,color=green!40]{{\bf Sergio: } #1}}


\newcommand{\obsbad}{\ensuremath{\hat{\mathbb{B}_o}}\xspace}
\newcommand{\obsall}{\ensuremath{\hat{\mathbb{T}_o}}\xspace}

\newcommand{\ignore}[1]{}

\newcommand{\xsub}[2]{\MVarNamed{#1}{#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Tikz Stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\tikzstyle{lastate}=[state,accepting,scale=0.3]
\tikzstyle{lainitial}=[initial,initial text={}, initial where=above]
\tikzstyle{lalabel}=[scale=1]

% Tikz directives for drawing HMM, PFSAs and other related macros
\tikzstyle{hmmstate}=[shape=circle,draw=blue!50,fill=blue!20]
\tikzstyle{hmminitialabove}=[initial,initial text={$I_\mathcal{H}:1$}, initial where=above]
\tikzstyle{hmminitialleft}=[initial,initial text={$I_\mathcal{H}:1$}, initial where=left]
\tikzstyle{hmminitialright}=[initial,initial text={$I_\mathcal{H}:1$}, initial where=right]
\tikzstyle{pfsainitial}=[initial,initial text={$I(x_1):1$}, initial where=above]
\tikzstyle{pfsainitialabove}=[initial,initial text={$I_\mathcal{A}:1$}, initial where=above]
\tikzstyle{pfsainitialleft}=[initial,initial text={$I_\mathcal{A}:1$}, initial where=left]
\tikzstyle{pfsainitialright}=[initial,initial text={$I_\mathcal{A}:1$}, initial where=right]
\tikzstyle{pfsafinal}=[hmmstate,accepting]
\tikzstyle{observation}=[shape=rectangle,draw=orange!50,fill=orange!20]
\tikzstyle{lightedge}=[<-,dotted]
\tikzstyle{mainstate}=[state,thick]
\tikzstyle{mainedge}=[<-,thick]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Listing Stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Syntax
\lstdefinelanguage{Enable}{
  morekeywords={let,in,if,then,else,new,bind,invoke,enable,disable,allow,disallow,fun,true,false,thk,event,callback,callin,force},
  literate={skip}{{$\bullet$}}1
}

\newcommand{\cbstyle}{\colordullx{0}\slshape}
\newcommand{\cistyle}{\colordullx{4}}
\newcommand{\fwktystyle}{\colordullx{1}\itshape\relsize{-1}}
\newcommand{\evtstyle}{\normalfont\ttfamily\scshape}
\lstdefinelanguage{exthighlighting}[]{highlighting}{%
  moredelim=**[is][\cbstyle]{|cb:}{|},
  moredelim=**[is][\cistyle]{|ci:}{|},
  moredelim=**[is][\fwktystyle]{|fwkty:}{|},
  moredelim=*[is][\evtstyle]{|evt:}{|}
}

\lstset{
  emphstyle=\cbstyle,
  emph={onCreate,onStart,onResume,onPause,onDestroy,onClick,onPrepared,onError,doInBackground,onPostExecute,onStop,onViewCreated,onCreateView,onCreateDialog},
  emphstyle={[2]\cistyle},
  emph={[2]setOnClickListener,setPositiveButton,setOnPreparedListener,reset,start,setEnabled,enable,disable,setDataSource,prepareAsync,execute,cancel,getResources,getWidth,dismiss,setContentView,show,getString,startActivity,setArguments,finish,add,show,findViewById,executeOnExecutor},
  emphstyle={[3]\fwktystyle},
  emph={[3]Activity,Activit,Button,AsyncTask,OnClickListener,View,Fragment,DialogFragment,AlertDialog,CountdownTimer,Dialog,PopupMenu,ListView,Toolbar},
  emphstyle={[4]\evtstyle},
  emph={[4]Create,Click,PostExecute},
  emphstyle={[5]\relsize{-1}\lstkeywordstyle},
  emph={[5]fwk,app}
}

\renewcommand{\lstkeywordstyle}{\relsize{-1}\fontseries{b}\selectfont}
\newcommand{\codej}[1]{\codex{language=Java,alsolanguage=exthighlighting}{#1}}
\newcommand{\coden}[1]{\codex{language=Enable,alsolanguage=exthighlighting}{#1}}
\newcommand{\enmkkw}[2]{\sbox#1{\coden{#2}}}
\newcommand{\codejmk}[3][\relax]{\sbox#2{#1\codej{#3}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Mathpartir and Arrays
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\arcr{\@arraycr}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Concrete Model
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\subst}[2]{\ensuremath{[#1/#2]}}

% Maps
\newcommand{\map}[1]{\ensuremath{[#1]}}
\newcommand{\maplet}[2]{\ensuremath{#1 \mathbin{\mapsto} #2}}
%\newcommand{\empmap}{\ensuremath{\map{\,}}}
\newcommand{\empmap}{\ensuremath{\cdot}}
\newcommand{\extmap}[1]{\ensuremath{{#1}}}
\newcommand{\MapST}[2]{\ensuremath{\left[\,#1 \SuchThat{#1}{#2} #2\,\right]}}

%%% Meta Variables
% 
\newcommand{\term}{\ensuremath{t}}
\newcommand{\expr}{\ensuremath{e}}
\newcommand{\ExprSet}{\SetName{Expr}}
\newcommand{\var}{\ensuremath{x}}
\newcommand{\VarSet}{\SetName{Var}}
\newcommand{\binding}[1]{\ensuremath{\theta_{#1}}}
\newcommand{\BindingSet}[0]{\ensuremath{\Theta}}
\newcommand{\applybind}[2]{\ensuremath{{#1}({#2})}}
\newcommand{\cont}{\ensuremath{k}}
\newcommand{\ContSet}{\SetName{Cont}}
\newcommand{\val}{\ensuremath{v}}
\newcommand{\ValSet}{\SetName{Val}}
\newcommand{\addr}{\ensuremath{a}}
\newcommand{\AddrSet}{\SetName{Addr}}
\newcommand{\thunk}{\ensuremath{\kappa}}
\newcommand{\thunkof}{\operatorname{thk}}
\newcommand{\ThunkSet}{\SetName{Thunk}}
\newcommand{\handle}{\ensuremath{h}}

%% Concrete syntax
\newcommand{\env}{\ensuremath{\eta}}
\newcommand{\EnvSet}{\SetName{Env}}
\newcommand{\store}{\ensuremath{\rho}}
\newcommand{\StoreSet}{\SetName{Store}}
\newcommand{\eventmap}{\ensuremath{\mu}}
\newcommand{\EventmapSet}{\SetName{Enabled}}
\newcommand{\callinmap}{\ensuremath{\nu}}
\newcommand{\CallinmapSet}{\SetName{Allowed}}

\newcommand{\fmtevt}[1]{\ensuremath{\text{\evtstyle #1}}}
\newcommand{\evtcb}[2]{\enFrame{\fmtevt{#1}}{#2}}

\newcommand{\stateconc}{\ensuremath{\sigma}}
\newcommand{\StateSet}{\SetName{State}}


\newsavebox{\@enkwLet}\enmkkw{\@enkwLet}{let}
\newcommand{\enkwLet}{\usebox{\@enkwLet}}
\newsavebox{\@enkwIn}\enmkkw{\@enkwIn}{in}
\newcommand{\enkwIn}{\usebox{\@enkwIn}}
\newsavebox{\@enkwIf}\enmkkw{\@enkwIf}{if}
\newcommand{\enkwIf}{\usebox{\@enkwIf}}
\newsavebox{\@enkwThen}\enmkkw{\@enkwThen}{then}
\newcommand{\enkwThen}{\usebox{\@enkwThen}}
\newsavebox{\@enkwElse}\enmkkw{\@enkwElse}{else}
\newcommand{\enkwElse}{\usebox{\@enkwElse}}
\newsavebox{\@enkwNew}\enmkkw{\@enkwNew}{new}
\newcommand{\enkwNew}{\usebox{\@enkwNew}}
\newsavebox{\@enkwBind}\enmkkw{\@enkwBind}{bind}
\newcommand{\enkwBind}{\usebox{\@enkwBind}}
\newsavebox{\@enkwInvoke}\enmkkw{\@enkwInvoke}{invoke}
\newcommand{\enkwInvoke}{\usebox{\@enkwInvoke}}
\newsavebox{\@enkwEnable}\enmkkw{\@enkwEnable}{enable}
\newcommand{\enkwEnable}{\usebox{\@enkwEnable}}
\newsavebox{\@enkwDisable}\enmkkw{\@enkwDisable}{disable}
\newcommand{\enkwDisable}{\usebox{\@enkwDisable}}
\newsavebox{\@enkwAllow}\enmkkw{\@enkwAllow}{allow}
\newcommand{\enkwAllow}{\usebox{\@enkwAllow}}
\newsavebox{\@enkwDisallow}\enmkkw{\@enkwDisallow}{disallow}
\newcommand{\enkwDisallow}{\usebox{\@enkwDisallow}}
\newsavebox{\@enkwFun}\enmkkw{\@enkwFun}{fun}
\newcommand{\enkwFun}{\usebox{\@enkwFun}}
\newsavebox{\@enkwForce}\enmkkw{\@enkwForce}{force}
\newcommand{\enkwForce}{\usebox{\@enkwForce}}
\newsavebox{\@enkwTrue}\enmkkw{\@enkwTrue}{true}
\newcommand{\enkwTrue}{\usebox{\@enkwTrue}}
\newsavebox{\@enkwFalse}\enmkkw{\@enkwFalse}{false}
\newcommand{\enkwFalse}{\usebox{\@enkwFalse}}
\newsavebox{\@enkwMe}\enmkkw{\@enkwMe}{thk}
\newcommand{\enkwMe}{\usebox{\@enkwMe}}
\newsavebox{\@enkwApp}\enmkkw{\@enkwApp}{app}
\newcommand{\enkwApp}{\usebox{\@enkwApp}}
\newsavebox{\@enkwFwk}\enmkkw{\@enkwFwk}{fwk}
\newcommand{\enkwFwk}{\usebox{\@enkwFwk}}
\newsavebox{\@enkwEvent}\enmkkw{\@enkwEvent}{event}
\newcommand{\enkwEvent}{\usebox{\@enkwEvent}}
\newsavebox{\@enkwCallback}\enmkkw{\@enkwCallback}{callback}
\newcommand{\enkwCallback}{\usebox{\@enkwCallback}}
\newsavebox{\@enkwCallin}\enmkkw{\@enkwCallin}{callin}
\newcommand{\enkwCallin}{\usebox{\@enkwCallin}}

\newcommand{\fmtstate}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\enkwDisallowed}{\fmtstate{bad}}
\newcommand{\enkwInitial}{\fmtstate{initial}}
\newcommand{\enkwFinal}{\fmtstate{final}}

\newcommand{\enLet}[3]{\ensuremath{\enkwLet\;#1\;\pcode{=}\;#2\;\enkwIn\;#3}}
\newcommand{\enGetf}[2]{\ensuremath{#1\pcode{.}#2}}
\newcommand{\enPutf}[3]{\ensuremath{#1\pcode{.}#2\;\pcode{=}\;#3}}
\newcommand{\enNew}{\enkwNew}
\newcommand{\enSkipK}{\ensuremath{\bullet}}
\newcommand{\enSkip}{\ensuremath{()}}
\newcommand{\enSeq}[2]{\ensuremath{#1\pcode{;}\,#2}}
\newcommand{\enIf}[3]{\ensuremath{\enkwIf\;#1\;\enkwThen\;#2\;\enkwElse\;#3}}
\newcommand{\enBind}[2]{\ensuremath{\enkwBind\;#1\;#2}}
%\newcommand{\enInvoke}[2]{\ensuremath{\enkwInvoke\;#1\;#2}}
\newcommand{\enInvoke}[1]{\ensuremath{\enkwInvoke\;#1}}
\newcommand{\enEnable}[1]{\ensuremath{\enkwEnable\;#1}}
\newcommand{\enDisable}[1]{\ensuremath{\enkwDisable\;#1}}
\newcommand{\enAllow}[1]{\ensuremath{\enkwAllow\;#1}}
\newcommand{\enDisallow}[1]{\ensuremath{\enkwDisallow\;#1}}
%\newcommand{\enFun}[3][\pkg]{\ensuremath{\enkwFun_{#1}\;#2\;\enkwIn\;#3}}
\newcommand{\enFun}[3][\pkg]{\ensuremath{#2\;\pcode{=>}_{#1}\;#3}}
\newcommand{\enForce}[1]{\ensuremath{\enkwForce\;#1}}
\newcommand{\enTrue}{\enkwTrue}
\newcommand{\enFalse}{\enkwFalse}
\newcommand{\enMe}{\ensuremath{\enkwMe}}
\newcommand{\enApp}{\enkwApp}
\newcommand{\enAppSub}{\ensuremath{\text{\tiny$\mathbf{in}$}}}
%\newcommand{\enAppSub}{\ensuremath{\shortleftarrow}}
\newcommand{\enFwk}{\enkwFwk}
%\newcommand{\enFwkSub}{\ensuremath{\text{\tiny$\mathbf{back}$}}}
\newcommand{\enFwkSub}{\ensuremath{\text{\tiny$\mathbf{bk}$}}}
%\newcommand{\enFwkSub}{\ensuremath{\shortrightarrow}}
%\newcommand{\enEvent}[1]{\ensuremath{\enkwEvent\;#1}}
%\newcommand{\enCallback}[1]{\ensuremath{\enkwCallback\;#1}}
%\newcommand{\enCallin}[1]{\ensuremath{\enkwCallin\;#1}}
\newcommand{\enEvent}{\enkwEvent}
\newcommand{\enCallin}{\enkwCallin}
\newcommand{\enInitial}{\enkwInitial}
\newcommand{\enDisallowed}{\enkwDisallowed}
\newcommand{\enDisallowedTrace}[1][\mword{}]{\enkwDisallowed\;#1}
\newcommand{\enCallback}{\enkwCallback}

%\newcommand{\enClosure}[2]{\ensuremath{#1[#2]}}
\newcommand{\enClosure}[2]{\ensuremath{#1}}

%\newcommand{\extMsg}[1]{\ensuremath{[#1]}}
%\newcommand{\extMsg}[1]{\ensuremath{\mathord{\triangleright}#1}}
\newcommand{\extMsg}[1]{\ensuremath{\mathord{;}#1}}

%\newcommand{\ext}[1]{\ensuremath{[#1]}}
\newcommand{\ext}[1]{\ensuremath{, #1}}
%\newcommand{\enMsg}[2]{\ensuremath{#1 #2}}
\newcommand{\enThunk}[2]{\ensuremath{#1[#2]}}
%\newcommand{\enThunk}[2]{\ensuremath{#1(#2)}}
\newcommand{\frameop}{\mathord{\gg}}
\newcommand{\enFrame}[2]{\ensuremath{#2\frameop#1}}
%\newcommand{\enLetK}[4]{\ensuremath{\enkwLet\;#1\;\pcode{=}\;#2\;\enkwIn\;#3}}
\newcommand{\enLetK}[4]{\ensuremath{#2 \triangleright #1.#3}}

%% Sergio: hide \store from the state
\newcommand{\@enState}{}
\long\def\@enState[#1][#2][#3][#4][#5][#6]{\ensuremath{\tuple{#1, #4, #5, #6}}}
\newcommand{\enState}{\optparams{\@enState}{[\expr][\env][\store][\eventmap][\callinmap][\cont]}}

\newcommand{\pkg}{\ensuremath{g}}
%\newcommand{\trans}{\ensuremath{\tau}}
\newcommand{\trans}{\ensuremath{\glabel{}}}
\newcommand{\transset}{\ensuremath{T}}
%\newcommand{\TransSet}{\SetName{Trans}}
\newcommand{\TransSet}{\GMsgSet}
\newcommand{\absTransSet}{\absofset{\TransSet}}

%%% Judgments
\newcommand{\jstep}[3][]{\ensuremath{#2 \longrightarrow_{#1} #3}}
\newcommand{\jstepins}[3][\trans]{\ensuremath{#2 \stackrel{\text{\normalsize$\longrightarrow$}}{\text{\scriptsize$#1$}} #3}}
\newcommand{\jstepnoins}[3][\trans]{\ensuremath{#2 \longrightarrow #3}}
\newcommand{\jcaption}[1]{\hfill\fbox{\normalsize$#1$}}



\newcommand{\obsty}{\MVar{fknd}}
\newcommand{\obstyret}{\MVar{rknd}}
\newcommand{\silentTrans}{\ensuremath{\cdot}}
\newcommand{\fmttrans}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\enkwInit}{\fmttrans{init}}
\newcommand{\enkwEvt}{\fmttrans{evt}}
\newcommand{\enkwCb}{\fmttrans{cb}}
\newcommand{\enkwCi}{\fmttrans{ci}}
\newcommand{\enkwDis}{\fmttrans{dis}}
\newcommand{\enkwRet}{\fmttrans{ret}}
%\newcommand{\enkwCbRet}{\fmttrans{cb^{\mathbf{return}}}}
%\newcommand{\enkwCiRet}{\fmttrans{ci^{\mathbf{return}}}}
\newcommand{\enkwCbRet}{\fmttrans{cbret}}
\newcommand{\enkwCiRet}{\fmttrans{ciret}}
\newcommand{\enkwFin}{\fmttrans{fin}}
\newcommand{\enObs}[2]{\ensuremath{#1\;#2}}
\newcommand{\enInit}{\fmttrans{init}}
\newcommand{\enEvt}[1]{\ensuremath{\enkwEvt\;#1}}
\newcommand{\enCb}[1]{\ensuremath{\enkwCb\;#1}}
\newcommand{\enCi}[1]{\ensuremath{\enkwCi\;#1}}
\newcommand{\enRetMsg}[2]{\ensuremath{#1\,\mathord{=}\,#2}}
\newcommand{\enCbRet}[2]{\ensuremath{\enRetMsg{#1}{\enkwCbRet\;#2}}}
\newcommand{\enCiRet}[2]{\ensuremath{\enRetMsg{#1}{\enkwCiRet\;#2}}}
\newcommand{\enDis}[1]{\ensuremath{\enkwDis\;#1}}
\newcommand{\enRet}[1]{\ensuremath{\enkwRet\;#1}}
\newcommand{\enFin}[1]{\ensuremath{\enkwFin\;#1}}
\newcommand{\Package}{\operatorname{pkg}}
\newcommand{\trace}{\ensuremath{\omega}}

% [SM] Eventually must disappear
\newcommand{\EnableSet}{\ensuremath{\overline{E}}}
% [SM] Eventually must disappear
\newcommand{\enablesymb}[1]{\ensuremath{b_{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Trace
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\FunSet}{\SetName{Fun}}
\newcommand{\fun}{\ensuremath{\lambda}}
\newcommand{\funinit}{\fun_{\mathbf{init}}}

% now it is ugly, we should change the syntax
\newcommand{\cbentry}[2]{\ensuremath{\enCb{#1[#2]}}}
\newcommand{\cbexit}[3]{\ensuremath{\enCbRet{#3}{#1[#2]}}}
\newcommand{\cientry}[2]{\ensuremath{\enCi{#1[#2]}}}
\newcommand{\ciexit}[3]{\ensuremath{\enCiRet{#3}{#1[#2]}}}
\newcommand{\params}{\ensuremath{p}}
\newcommand{\retval}{\ensuremath{r}}

\newcommand{\rtrace}[1]{\ensuremath{\tau_{#1}}}
\newcommand{\rtracecb}[1]{{\trace_{#1}}}
\newcommand{\rtraceci}[1]{{\trace{#1}}^{CI}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Abstraction
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% ground
\newcommand{\ground}[1]{\ensuremath{{#1}}}
\newcommand{\GMsgSet}{\ensuremath{{\Sigma}}}
\newcommand{\GMsgSetFwk}{\ensuremath{{\Sigma^{\enFwkSub}}}}
\newcommand{\GMsgSetApp}{\ensuremath{{\Sigma^{\enAppSub}}}}
\newcommand{\glabel}[1]{\ensuremath{{\ground{m}}_{#1}}}
\newcommand{\glabelFwk}[1]{\ensuremath{\ground{m^{\enFwkSub}}}_{#1}}
\newcommand{\glabelApp}[1]{\ensuremath{\ground{m^{\enAppSub}}}_{#1}}

\newcommand{\myabs}[1]{\ensuremath{\hat{#1}}}
\newcommand{\perset}{\ensuremath{\myabs{\mu}}}
\newcommand{\proset}{\ensuremath{\myabs{\nu}}}

\newcommand{\persetinit}{\perset^{\initsub}_{\rspec{}}}
\newcommand{\prosetinit}{\proset^{\initsub}_{\rspec{}}}

\newcommand{\errorstate}{\ensuremath{\myabs{}}}
\newcommand{\absstate}{\ensuremath{\myabs{\sigma}}}
\newcommand{\AbsStateSet}{\SetName{AbsState}}
\newcommand{\@enAbsState}{}
\long\def\@enAbsState[#1][#2][#3]{\ensuremath{\tuple{#1, #2, #3}}}
\newcommand{\enAbsState}{\optparams{\@enAbsState}{[\perset][\proset][\trace]}}
\newcommand{\mpath}{\ensuremath{{{\myabs{\pi}}}}}
\newcommand{\mpathsubs}[1]{\ensuremath{{{\myabs{\pi}_{{#1}}}}}}
%\newcommand{\othermodel}{lifecycle$++$}
%\newcommand{\Othermodel}{Lifecycle$++$}
\newcommand{\othermodel}{\lifecyclepp}
\newcommand{\Othermodel}{\Lifecyclepp}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Spec language
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\newcommand{\parstyle}[1]{\ensuremath{{\boldsymbol{#1}}}}
\newcommand{\PMsgSet}{\ensuremath{\SetName{\parstyle{\Sigma}}}}
\newcommand{\PMsgSetFwk}{\ensuremath{\SetName{\parstyle{\Sigma_{\enFwkSub}}}}}
\newcommand{\PMsgSetApp}{\ensuremath{\SetName{\parstyle{\Sigma_{\enAppSub}}}}}
\newcommand{\mlabel}[1]{\ensuremath{\parstyle{m_{#1}}}}
\newcommand{\mlabelFwk}[1]{\ensuremath{\parstyle{m^{\enFwkSub}}}_{#1}}
\newcommand{\mlabelApp}[1]{\ensuremath{\parstyle{m^{\enAppSub}}}_{#1}}
\newcommand{\mparams}{\ensuremath{\parstyle{\params}}}
\newcommand{\mretval}{\ensuremath{\parstyle{r}}}

\newcommand{\specvar}{\ensuremath{\ell}}
\newcommand{\SpecVarSet}{\SetName{SVar}}

\newcommand{\mstate}[1]{\ensuremath{\absstate_{{#1}}}}
\newcommand{\mpathlength}[1]{\ensuremath{k_{#1}}}
\newcommand{\length}[1]{\ensuremath{|{#1}|}}

\newcommand{\mword}[1]{\ensuremath{\omega_{{#1}}}}

\newcommand{\prefix}[3]{\ensuremath{{#1}_{#3}^{{#2}..}}}
\newcommand{\mpathstate}[3]{\ensuremath{{#1}_{#3}^{{#2}..{#2}}}}

\newcommand{\suffix}[3]{\ensuremath{{#1}_{#3}^{..{#2}}}}

\newcommand{\rrule}[1]{\ensuremath{\parstyle{s_{#1}}}}
\newcommand{\rspec}[1]{\ensuremath{\parstyle{S_{#1}}}}

\newcommand{\grrule}[1]{\ensuremath{s_{#1}}}
\newcommand{\grspec}[1]{\ensuremath{S_{#1}}}

\newcommand{\renable}{\ensuremath{\rightarrow}}
\newcommand{\rdisable}{\ensuremath{\nrightarrow}}
\newcommand{\rregexp}[1]{\ensuremath{\parstyle{r_{#1}}}}
\newcommand{\grregexp}[1]{\ensuremath{r_{#1}}}

\newcommand{\emptyword}{\ensuremath{\epsilon}}
\newcommand{\falseword}{\ensuremath{\emptyset}}
\newcommand{\rseq}{\ensuremath{;}}
\newcommand{\rstar}{\ensuremath{^{*}}}
\newcommand{\rand}{\ensuremath{\cap}}
\newcommand{\ror}{\ensuremath{+}}
\newcommand{\rnot}{\ensuremath{\neg}}

\newcommand{\truestar}{\ensuremath{\GMsgSet \rstar}}
\newcommand{\change}[4]{\ensuremath{\textit{notchange}({#1},{#2},{#3},{#4})}}
\newcommand{\enable}[4]{\ensuremath{\textit{enable}({#1},{#2},{#3},{#4})}}
\newcommand{\disable}[4]{\ensuremath{\textit{disable}({#1},{#2},{#3},{#4})}}

\newcommand{\updatename}[2]{\operatorname{upd}^{#1}_{#2}}
%%\newcommand{\updatename}[2]{\ensuremath{\smash{\phi^{#1}_{#2}}}}
\newcommand{\evalFwk}[3]{\ensuremath{\updatename{\enFwkSub}{#2}({#3},{#1})}}
\newcommand{\evalApp}[3]{\ensuremath{\updatename{\enAppSub}{#2}({#3},{#1})}}
%% \newcommand{\evalFwk}[3]{\ensuremath{\updatename{\enFwkSub}{#2}({#3},{#1})}}
%% \newcommand{\evalApp}[3]{\ensuremath{\updatename{\enAppSub}{#2}({#3},{#1})}}
%% \newcommand{\evalFwk}[3]{\ensuremath{\operatorname{updback}_{#2}({#3},{#1})}}
%% \newcommand{\evalApp}[3]{\ensuremath{\operatorname{updin}_{#2}({#3},{#1})}}


\newcommand{\SpecPaths}[1]{\ensuremath{\denote{#1}}}
\newcommand{\FunFwkSet}{\ensuremath{\FunSet_{\enkwFwk}}}
\newcommand{\FwkImpl}{\ensuremath{\tuple{\FunFwkSet,\funinit}}}

\newcommand{\permit}[3]{\ensuremath{\operatorname{permit}_{#1}({#2},{#3})}}
\newcommand{\prohibit}[3]{\ensuremath{\operatorname{prohibit}_{#1}({#2},{#3})}}
\newcommand{\consistent}[2]{\ensuremath{\operatorname{consistent}_{#1}({#2})}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Dynamic verification
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tracerepetitions}{\traceset{(\rtracecb{1} \ror \ldots \ror \rtracecb{l}) \rstar{}}}
\newcommand{\subtraceset}[1]{\ensuremath{Sub_{#1}}}
\newcommand{\repetitions}[2]{\ensuremath{\Omega_{{#1},{#2}}}}

\newcommand{\GMsgSetTrace}[1]{\ensuremath{\ground{\Sigma_{#1}}}}
\newcommand{\GMsgSetTraceFwk}[1]{\ensuremath{\GMsgSetTrace{#1}^{\enFwkSub}}}
\newcommand{\GMsgSetTraceApp}[1]{\ensuremath{\GMsgSetTrace{#1}^{\enAppSub}}}

\newcommand{\PMsgSetTrace}[1]{\ensuremath{\parstyle{{\Sigma_{#1}}}}}
\newcommand{\BindingSetTrace}[2]{\ensuremath{\ground{\BindingSet_{{#1},{#2}}}}}

\newcommand{\tsm}[1]{\ensuremath{M_{#1}}}
\newcommand{\tsvar}[1]{\ensuremath{X_{#1}}}
\newcommand{\tsinit}[1]{\ensuremath{I_{#1}}}
\newcommand{\tstrans}[1]{\ensuremath{T_{#1}}}
\newcommand{\prop}[1]{\ensuremath{P_{#1}}}
\newcommand{\tspath}[1]{\ensuremath{\pi}}
\newcommand{\tssync}[2]{\ensuremath{{#1} | {#2}}}

\newcommand{\accepting}[1]{\ensuremath{\text{Acc}_{#1}}}
\newcommand{\effect}[1]{\ensuremath{\text{Update}_{\grrule{#1}}}}

\newcommand{\commonvar}{\tsvar{ABS}}
\newcommand{\msgvar}{\ensuremath{l}}
\newcommand{\dom}[1]{\ensuremath{Dom({#1})}}
\newcommand{\pcvar}{\ensuremath{pc}}

\newcommand{\errstate}{\ensuremath{error}}
\newcommand{\sinkstate}{\ensuremath{sink}}
\newcommand{\offset}[1]{\ensuremath{o_{#1}}}

\newcommand{\singlemsg}[3]{\ensuremath{u_{{#1},{#2},{#3}}}}

%%% Spec Arrows
%\newcommand{\specArrow}{\mathord{\shortrightarrow}}
%\newcommand{\specArrow}{\mathord{\rightarrow}}
%\newcommand{\nspecArrow}{\mathord{\nrightarrow}}
\newcommand{\specArrow}{\mathord{\rightarrowtriangle}}
\newcommand{\nspecArrow}{\mathord{\not\rightarrowtriangle}}
%\newcommand{\specEnableOp}{\mathop{\diamondplus}}
\newcommand{\specEnableOp}{\mathop{\text{\relsize{-1}\enkwEvt}}}
%\newcommand{\specDisableOp}{\mathop{\diamondminus}}
\newcommand{\specDisableOp}{\mathop{\text{\relsize{-1}\enkwEvt}}}
%\newcommand{\specAllowOp}{\mathop{\boxplus}}
\newcommand{\specAllowOp}{\mathop{\text{\relsize{-1}\enkwCi}}}
%\newcommand{\specDisallowOp}{\mathop{\boxminus}}
\newcommand{\specDisallowOp}{\mathop{\text{\relsize{-1}\enkwCi}}}

\newcommand{\specEnable}[3][]{\ensuremath{#2 \specArrow_{#1} \specEnableOp #3}}
\newcommand{\specDisable}[3][]{\ensuremath{#2 \nspecArrow_{#1} \specDisableOp #3}}
\newcommand{\specAllow}[3][]{\ensuremath{#2 \specArrow_{#1} \specAllowOp #3}}
\newcommand{\specDisallow}[3][]{\ensuremath{#2 \nspecArrow_{#1} \specDisallowOp #3}}

\newcommand{\allSpecs}[4]{\ensuremath{{#3}_{\joinrel{#1}{#2}}(#4)}}
\newcommand{\allEnables}[1]{\allSpecs{\specArrow}{\specEnableOp}{}{#1}}
\newcommand{\allDisables}[1]{\allSpecs{\nspecArrow}{\specDisableOp}{}{#1}}
\newcommand{\allAllows}[1]{\allSpecs{\specArrow}{\specAllowOp}{}{#1}}
\newcommand{\allDisallows}[1]{\allSpecs{\nspecArrow}{\specDisallowOp}{}{#1}}
\newcommand{\allRules}[1]{\allSpecs{\dashrightarrow}{}{}{#1}}

\newcommand{\specPermit}[3][]{\ensuremath{#2 \specArrow_{#1} #3}}
\newcommand{\specForbid}[3][]{\ensuremath{#2 \nspecArrow_{#1} #3}}

\newcommand{\traceset}[1]{\llbracket #1 \rrbracket}
%\newcommand{\traceset}[1]{\ensuremath{\Omega_{#1}}}
\renewcommand{\denote}[1]{\operatorname{paths}(#1)}

\newcommand{\initsub}{\text{\rm init}}

\makeatother

